MinTL: Minimalist Transfer Learning for Task-Oriented Dialogue Systems

In this paper, we propose Minimalist Transfer Learning (MinTL) to simplify the system design process of task-oriented dialogue systems and alleviate the over-dependency on annotated data. MinTL is a simple yet effective transfer learning framework, which allows us to plug-and-play pre-trained seq2seq models, and jointly learn dialogue state tracking and dialogue response generation. Unlike previous approaches, which use a copy mechanism to "carryover" the old dialogue states to the new one, we introduce Levenshtein belief spans (Lev), that allows efficient dialogue state tracking with a minimal generation length. We instantiate our learning framework with two pre-trained backbones: T5 and BART, and evaluate them on MultiWOZ. Extensive experiments demonstrate that: 1) our systems establish new state-of-the-art results on end-to-end response generation, 2) MinTL-based systems are more robust than baseline methods in the low resource setting, and they achieve competitive results with only 20\% training data, and 3) Lev greatly improves the inference efficiency.

==> figure_OLD.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,420); %set diagram left start at 0, and has height of 420

%Rounded Rect [id:dp4397180179071407] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=0.79 ] (235,76.6) .. controls (235,71.85) and (238.85,68) .. (243.6,68) -- (272.33,68) .. controls (277.08,68) and (280.93,71.85) .. (280.93,76.6) -- (280.93,102.4) .. controls (280.93,107.15) and (277.08,111) .. (272.33,111) -- (243.6,111) .. controls (238.85,111) and (235,107.15) .. (235,102.4) -- cycle ;
%Straight Lines [id:da14950354489996975] 
\draw    (205.5,100) -- (230,100) ;
\draw [shift={(233,100)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da7898645800998412] 
\draw    (396.67,113.67) -- (396.56,136.37) ;
\draw [shift={(396.54,139.37)}, rotate = 270.27] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da25578318377899434] 
\draw    (206.5,80) -- (231,80) ;
\draw [shift={(234,80)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Rounded Rect [id:dp23328318043248863] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.48 ] (374,76.6) .. controls (374,71.85) and (377.85,68) .. (382.6,68) -- (411.33,68) .. controls (416.08,68) and (419.93,71.85) .. (419.93,76.6) -- (419.93,102.4) .. controls (419.93,107.15) and (416.08,111) .. (411.33,111) -- (382.6,111) .. controls (377.85,111) and (374,107.15) .. (374,102.4) -- cycle ;
%Straight Lines [id:da6186018923496734] 
\draw    (284.93,90) -- (368,90) ;
\draw [shift={(371,90)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Rounded Rect [id:dp38288232855160476] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.48 ] (235,199.6) .. controls (235,194.85) and (238.85,191) .. (243.6,191) -- (272.33,191) .. controls (277.08,191) and (280.93,194.85) .. (280.93,199.6) -- (280.93,225.4) .. controls (280.93,230.15) and (277.08,234) .. (272.33,234) -- (243.6,234) .. controls (238.85,234) and (235,230.15) .. (235,225.4) -- cycle ;
%Straight Lines [id:da04708028146220555] 
\draw    (257.93,115.57) -- (257.93,184) ;
\draw [shift={(257.93,187)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da7472375007722889] 
\draw    (230.41,211.17) -- (208.41,211.17) ;
\draw [shift={(205.41,211.17)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Flowchart: Magnetic Disk [id:dp7161234701534951] 
\draw   (413,199.78) -- (413,221.23) .. controls (413,224.41) and (405.6,227) .. (396.46,227) .. controls (387.33,227) and (379.93,224.41) .. (379.93,221.23) -- (379.93,199.78)(413,199.78) .. controls (413,202.96) and (405.6,205.55) .. (396.46,205.55) .. controls (387.33,205.55) and (379.93,202.96) .. (379.93,199.78) .. controls (379.93,196.59) and (387.33,194) .. (396.46,194) .. controls (405.6,194) and (413,196.59) .. (413,199.78) -- cycle ;
%Straight Lines [id:da08775709653821528] 
\draw    (396.59,166.29) -- (396.48,189) ;
\draw [shift={(396.46,192)}, rotate = 270.27] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da5399568188356916] 
\draw    (373.93,211) -- (346.41,211.15) ;
\draw [shift={(343.41,211.17)}, rotate = 359.68] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Square [id:dp645811675827052] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (335.57,196.93) -- (335.57,207) -- (325.5,207) -- (325.5,196.93) -- cycle ;
%Shape: Square [id:dp05185048123636693] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (335.57,206.93) -- (335.57,217) -- (325.5,217) -- (325.5,206.93) -- cycle ;
%Shape: Square [id:dp6974452857946962] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (335.57,216.93) -- (335.57,227) -- (325.5,227) -- (325.5,216.93) -- cycle ;
%Straight Lines [id:da9682787629709972] 
\draw    (316.93,211) -- (289.41,211.15) ;
\draw [shift={(286.41,211.17)}, rotate = 359.68] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

% Text Node
\draw (174,70) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$B_{t-1}$};
% Text Node
\draw (241,80.6) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\mathbf{Enc}$};
% Text Node
\draw (326,142) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$B_{t} =f( \mathcolorbox{soulbleu}{Lev_{t}} ,B_{t-1})$};
% Text Node
\draw (180,90) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$C_{t}$};
% Text Node
\draw  [color={rgb, 255:red, 255; green, 255; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (314,77) -- (335,77) -- (335,101) -- (314,101) -- cycle  ;
\draw (318,83) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$H$};
% Text Node
\draw (378,80.6) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\mathbf{Dec}_{L}$};
% Text Node
\draw  [color={rgb, 255:red, 255; green, 255; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (247,135) -- (268,135) -- (268,159) -- (247,159) -- cycle  ;
\draw (248,140) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$H$};
% Text Node
\draw (237,203.5) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\mathbf{Dec}_{R}$};
% Text Node
\draw (184,202) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$R_{t}$};
% Text Node
\draw (381,208) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\mathbf{KB}$};


\end{tikzpicture}

